A Survey of HTTPS Traffic and Services Identification Approaches

HTTPS is quickly rising alongside the need of Internet users to benefit from security and privacy when accessing the Web, and it becomes the predominant application protocol on the Internet. This migration towards a secure Web using HTTPS comes with important challenges related to the management of HTTPS traffic to guarantee basic network properties such as security, QoS, reliability, etc. But encryption undermines the effectiveness of standard monitoring techniques and makes it difficult for ISPs and network administrators to properly identify and manage the services behind HTTPS traffic. This survey details the techniques used to monitor HTTPS traffic, from the most basic level of protocol identification (TLS, HTTPS), to the finest identification of precise services. We show that protocol identification is well mastered while more precise levels keep being challenging despite recent advances. We also describe practical solutions that lead us to discuss the trade-off between security and privacy and the research directions to guarantee both of them.

==> detect-ssl.tex <==
\begin{algorithm}
   \caption{Detect Server-Hello Packet - From \cite{Bernaille2007}}
   \setlength{\belowcaptionskip}{-5pt}
   \label{ssl-detect}
    \begin{algorithmic}[1]
    	\If {$bit_{2}[0]=1$ and $bit_{2}[1]=0$ and $bit_{2}[2:15]= Size_{2}$ and $Byte_{2}[3]=4$}
    		\State Connection is an SSLv2 connection
		 \ElsIf {$Byte_{2}[1]=22$ and $Byte_{2}[2]=3$}
		 	\If {$ Byte_{2}[3]=0$}
		 		\State Connection is an SSLv3.0 connection
		 	\ElsIf {$Byte_{2}[3] = 1$}
		 		\State Connection is a TLS connection
		 	\Else 
		 		\State Connection is not using SSL
		 	\EndIf
		\Else 
			\State Connection is not using SSL
    	\EndIf 
\end{algorithmic}
\end{algorithm}
 

==> discussion.tex <==
In the above sections, we notice that there are increased demands for privacy sensitive methods to monitor and control HTTPS traffic. Such demands create a paradox between security and privacy. The answer to this conflict is not easy, as both sides are valuable factors over Internet. After Snowden affair this issue is named "Dilemmas of the Internet age"  , which has been discussed not only in the academic community but also it has been extended to democracy and human rights space. %The European Court of Human Rights (ECtHR) implied the monitoring of personal Internet usage by \textit{"analysis of the websites visited, the times and dates of the visits to the websites and their duration"} \cite{stalla2013online}. 
Author in \cite{caloyannides2004privacy} discusse the statement that \textit{"To prevent terrorism (or spam, or cyber-crime, or male-pattern baldness, or whatever one dreads), we must empower police to monitor all online activities"}. Author claim such monitoring activities are ineffective as they may identify some trivial crime, but they can not recognize professional criminals or the persons well educated in working under surveillance. 

An important argument arise if massive online monitoring takes place how we trust people work on, and how to guarantee that an administration in power won't abuse the intercepted information to intimidate its opponents. Author conclude that if online monitoring may fix a problem, but it can create even more serious problems. 

Enterprise owners may have good arguments for monitoring and filtering access to their network. Beside security reasons,  statistics show that 44\% of online video is being viewed during work time and even 29\% of accessed adult websites are from work computers. Monitoring can be worthy since the wasted time could impact employees productivity \cite{currentware}.Monitoring can be worthy since the wasted time could impact employees productivity \cite{currentware}.  
Moreover, the company is the owner of the network. However, is it sufficient to legitimate exposition of employees private data with HTTPS proxy?

The Cyber-security Research Ethics Dialog\& Strategy Workshop started in 2013, the discussion about the impact of cyber-security research on infrastructure security, network neutrality, free market competition, technology transfer and intellectual property rights \cite{Velan2015}. To conclude, we think that the best solution is to pursue the goal of techniques identifying HTTPS services without decryption. The research community must work on techniques offering both security and privacy.
